A New Coreset Framework for Clustering

Given a metric space, the $(k,z)$-clustering problem consists of finding $k$ centers such that the sum of the of distances raised to the power $z$ of every point to its closest center is minimized. This encapsulates the famous $k$-median ($z=1$) and $k$-means ($z=2$) clustering problems. Designing small-space sketches of the data that approximately preserves the cost of the solutions, also known as \emph{coresets}, has been an important research direction over the last 15 years. In this paper, we present a new, simple coreset framework that simultaneously improves upon the best known bounds for a large variety of settings, ranging from Euclidean space, doubling metric, minor-free metric, and the general metric cases.

==> centroid-minor.tex <==
\subsection{In Minor-Excluded Graphs} \label{sec:centroid-minor}

A graph $H$ is a \textit{minor} of a graph $G$ if it can be obtained from $G$ by deleting edges and vertices and contracting edges. 

We are interested here in families of graph excluding a fixed minor $H$, i.e. none of the graph in the family contains $H$ as a minor. Those graphs are weighted: we assume that for each edge, its value is equal to shortest-path distance between its two endpoints.

The goal of this section is to prove the following lemma, analogous to \cref{lem:centroid-treewidth}. 


\begin{lemma}\label{thm:mf-centroid}
  Let $G = (V, E)$ be an edge-weighted graph that excludes a fixed minor, a set $X \subseteq V$ and two positive integers $k$ and $z$. Furthermore, let $\greedy$ be a solution of $(k, z)$-clustering of $X$. 
  
  There exists a set $\cand$ of size $\exp(O(\log^2 |X| + \log |X| / \eps^4))$ with the following property.
  
  For every set $\calS$ of $k$ centers, there exists $\tilde \calS \in \cand^k$ such that for all points $p \in X$ such that either $\cost(p, \calS) \leq \left(\frac{8z}{\eps}\right)^z \cost(p, \greedy)$ or $\cost(p, \tilde \calS) \leq \left(\frac{8z}{\eps}\right)^z \cost(p, \greedy)$, 
\[|\cost(p, \calS) - \cost(p, \tilde{\calS})| \leq \eps^3 \left(\cost(p, \calS) + \cost(p, \greedy)\right).\]
\end{lemma}

As for treewidth, this lemma implies the following corollary:

\begin{corollary}
\label{cor:coreset-minor}
  Let $G = (V, E)$ be an edge-weighted graph that excludes a fixed minor, and two positive integers $k$ and $z$ . 
  
  There exists an algorithm with running time $\tilde O(nk)$ that constructs an $\eps$-coreset for $(k, z)$-clustering on $V$ with size 
  \[O\left(\frac{\log^5 1/\eps}{2^{O(z\log z)}\min(\eps^3, \eps^z)}\left(k \log^2 k \log(1/\eps) + \frac{k \log k}{\eps^4} + \log 1/\pi\right)\right)\]
\end{corollary}


The big picture is the same as for treewidth. Minor-free graphs have somewhat nice separators, that we can use to select centers. However, those separators do not have bounded size: they are instead made of a bounded number of shortest path, as described in the next structural lemma.

\begin{lemma}[Balanced Shortest Path Separator~\cite{AbrahamG06}]
    \label{lem:mf_sp_sep}
    Given a graph $G=(V, E)$ with positive weights on vertices and that excludes a fixed minor,
    there is a set of vertices $S \subseteq V$, such that
    \begin{enumerate}
        \item $S = P_1 \cup P_2 \cup \ldots$ where $P_i$ is a set of shortest
        paths in the graph formed by removing $\bigcup_{j < i}{P_j}$
        \item $\sum_{i}{|P_i|} = O(1)$, where the hidden constant depends on the size of the excluded minor
        \item the weight of every component in the graph
        formed by removing $S$ from $G$ is at most half the weight of $V$.
    \end{enumerate}
\end{lemma}


Applying recursively that lemma on the graph $G$ with weight $1$ for vertices in $X$ and $0$ otherwise yields a recursive decomposition $\calR$ (see \cite{braverman20minor} for more details about that decomposition).

The general sketch of the proof for $z=1$ is as follows: in every leaf of $\calR$, we would like to take a net, approximating well every center lying in the leaf. Unfortunately, small nets do not exist in minor-free graphs. To cope with that issue, we proceed slightly differently, inspired by \cite{Cohen-AddadPP19, braverman20minor}: in short, we consider the boundary $B$ of the leaf, and enumerate all possible tuple of distances from a point inside the leaf to the boundary. For each tuple, we include in $\cand$ a point realizing it. Of course, this would lead to a set $\cand$ way too big: the boundary of each leaf consists of too many points, and there are too many distances possible. For that, we show how to discretize the boundary by placing \emph{landmarks} on it, and how to round distances from a point to a landmark.

We first picture how to discretize the boundary. Let $S$ be a cluster with center $s$ of the solution $\calS$. Let $p \in S$ be a tiny or interesting point, and $R$ the smallest region of $\calR$ containing both $y$ and $s$. Let $P_1, P_2, ..., P_m$ the set of shortest paths given by the application of \cref{lem:mf_sp_sep} on $R$. Removing all those path separates $p$ and $s$: hence, the path $y \leadsto s$ must cross a path in some $P_i$. Let $i$ be the smallest index such that $p \leadsto s$ intersects a path $P\in P_i$. Let $x$ be the intersecting point. If there where a landmark $l$ close to $x$, we could write:
\begin{eqnarray*}
\dist(p, s) = \dist(p, x) + \dist(x, s) \approx \dist(y, l) + \dist(l, s)\\
 = \dist(p, l) + \dist(l, \tilde s) \geq \dist(y, \tilde s)
\end{eqnarray*}
where $\tilde s \in \cand$ is the point realizing the same distance to the landmarks as $s$. Similarly, one can show $\dist(p, \tilde s) \gtrapprox \dist(p, s)$, so $\dist(p, s) \approx \dist(p, \tilde s)$ which would be enough to conclude. We list some properties that will help us to find landmarks. First, $P$ is a shortest path in $R_j := R \setminus \cup_{j < i} P_i$. 
Additionally, $x$ is at distance at most $\dist(y, s) \leq \dist(y, \greedy)/\eps$ of $p$, since $p$ is of type tiny or interesting. Hence, the landmarks could be a $\eps \dist(y, \greedy)$-net of $P \cap B_{R_j}(y, \eps^{-2}\dist(y, \greedy))$: this would ensure that there is a landmark close to the $p$-to-$s$ path, allowing to write the previous line of equalities. Note as well that this net has constant size.

However, $\tilde s$ must be chosen consistently for every possible $p$, and so the landmarks must be the same for all $p \in S$. For this, focus first on the $p$ separated from $s$ by the path $P$, to construct a consistent set of landmarks. Among them, let $p_0$ with smallest $\dist(p, \greedy)$ value.
%with smallest $\Delta_{C_y}$ value. 
Every other $p$ that intersect $P$ in $B_{R_j}(p_0, \eps^{-2}\dist(p_0, \greedy))$ is taken care of by landmarks defined for $p_0$. 
In particular, $p$ such that $\dist(p, s) \leq \eps^{-2}\dist(p_0, \greedy) \leq \eps^{-2}\dist(p, \greedy)$ are fine. 
In the case where $\dist(p, s) > \eps^{-2}\dist(p_0, \greedy)$, then we can argue that $\dist(s, \tilde s)$ is tiny compared to $\dist(p,s)$: 
indeed, since $\tilde s$ has the same distances to landmarks than $s$, it must be that $d(p_0, \tilde s) \approx d(p_0, s)$. 
Hence, $\dist(s, \tilde s) \leq \dist(s, p_0) + \dist(\tilde s, p_0) \lessapprox 2 \eps^{-2}\dist(p_0, \greedy) \leq 2 \eps \dist(p, s)$ and finally $|d(p, \tilde s) - \dist(p, s)|\leq 2\eps\dist(p, s)$.

This argument works for all $p$ separated from $s$ by the same path. To ensure consistency over all $p$, we pick one $p_0$ for every possible such path, and choose $\tilde s$ to have the same distances as $s$ to all those $p_0$.

We make now the proof formal, and work for all powers $z$.

%\david{For the size: $s$ is in at most $O(\log |X|)$ regions (the depth of the decomposition), in each of them we consider $O(1)$ paths, and consider $1/\eps^2$ landmarks for each of them. There are thus $|X|^{O(\log |X|)} \cdot O(1) \cdot 1/\eps^2$ possible set of landmarks. Furthermore, each of these set contains $O(\log |X| \poly(1/\eps))$ portals. Since the distance from $s$ to a landmark defined by a point $y$ is at most $\eps^{-3}\Delta_{C_{p_0}}$ and the error allowed for those points is $\eps\Delta_{C_{y}}$, there are $1/\eps^4$ possible distance to any landmark, and hence a given set of landmarks yields $(1/\eps)^{O(\log |X| \poly(1/\eps))}$ many distance interface. So in total, $|\cand|=(1/\eps)^{O(\log |X| \poly(1/\eps))} \cdot |X|^{O(\log |X|)} \cdot 1/\eps^2 = \exp(\poly(\log (|X|)/\eps))$}

\begin{proof}[Proof of \cref{thm:mf-centroid}]
  Consider a recursive decomposition $\calR$ of the graph, i.e. a tree where each tree node is a subset of $V$, and where a node is equal to the union of its children. 
  In our case, $\calR$ is constructed as follows. The root node is the whole vertex set. Then, inductively, apply Lemma \ref{lem:mf_sp_sep}, with weights $1$ on vertices of $X$ and $0$ otherwise,
  on a region $R$ represented by a node (simply called region in the following): the children of $R$ are
\begin{itemize}
\item the connected components of $R \setminus S$,
\item let $S = P_1 \cup P_2 \cup ...$. Each path in $P_i$ is broken into maximal subpath each containing a point of $X$, and each subpath is added as a children of $R$.
\end{itemize}
Stop this induction when a region has weight at most 2 (i.e., there are less than 2 nodes from $X$ in it).
Since the weight is divided by two at every level, the depth of that decomposition is $O(\log |X|)$.

We define sets of landmarks as follows. Consider a root-to-leaf path of the decomposition $R_1, ..., R_{\log |X|}$. Let $P^i_1, P^i_2 ...$ be the paths given by Lemma \ref{lem:mf_sp_sep} on $R_i$.
For each of those paths, choose a vertex $p^i_j \in R_i$ and let $\calL_{i, j, p^i_j}$ be an $\frac{\epsilon}{z}  \dist(p^i_j, \greedy)$-net of $P \cap B_{R^j_i}(p^i_j,  \frac{90z^3}{\eps^3}\dist(p^i_j, \greedy))$, 
where $B_{R^j_i}(y, r)$ is the ball centered at $y$ of radius $r$ in the graph $R^j_i$, which is the graph induced by $R_i \setminus \bigcup_{j' \leq j} P^i_{j'}$.

We let $\by$ be any such sequence $p^1_1, p^1_2, ..., p^2_1, p^2_2,...$, where $p^i_j \in R_i$ for all path $P^i_j$ dividing $R_i$. A set of landmarks $\calL_{\by}$ is defined as:
\[\calL_\by := \big(X \cap R_{\log |X|}\big) \bigcup_{i,j} \calL_{i,j, p^i_j}.\]



We now describe how we round distances to landmarks, and argue that for each possible distance tuple, $\cand$ contains a point having that distance tuple.
Formally, given a point $p$ and its distance tuple $\mathbf{d}(p) = (\dist(p, x)~ | ~\forall~x\in X \cap R_{\log |X|}) + (\dist(p, y)~ |~ y \in \calL_{i,j,p^i_j}, \forall i,j)$,
the \emph{rounded distance tuple} $\tilde{\mathbf{d}}(p)$ is defined as follows
:
\begin{itemize}
\item For $x \in X \cap A$, $\tilde d(p, x)$ is the multiple of 
$\frac{\eps}{z} \dist(x, \greedy)$ smaller than $\frac{8z}{\eps} \dist(x, \greedy)$ closest to $\dist(p, x)$. 
\item For $y \in \calL_{i,j,p^i_j}$, $\tilde d(p, y)$  is the multiple of 
$\frac{\eps}{z}\cdot \cost(p^i_j, \greedy)$ smaller than $\frac{90z^3}{\eps^3}\cost(p^i_j, \greedy)$ closest to $\dist(p, y)$. 
\end{itemize}

The set $\cand$ is constructed as follows: for every root-to-leaf path and every sequence $\by$, for every rounded distance tuple $\{\tilde{\mathbf{d}}(p)\}$, add to $\cand$ a point that realizes this rounded distance tuple.

It remains to show both that $\cand$ has size $\exp(\poly(\log (|X|)/\eps))$, and that $\cand$ contains good approximation of each center of any given solution.

\paragraph*{Size analysis.}
$\cand$ contains one point per rounded distance tuple. 
For a given set of landmarks $\calL_\by$, there are $\left(\frac{90z^4}{\eps^4}\right)^{|\calL_\by|}$ possible rounded distances. Since the decomposition has depth $\log |X|$ and there is $O(1)$ paths for each region as prescribed by Lemma \ref{lem:mf_sp_sep}, there are $O(\log |X|)$ paths $P^i_j$; for each of them, there are $O(1/\eps^4)$ landmarks (the size of the net). Hence, $|\calL_\by| = O(\log(|X|)/\eps^{4})$. 

The number of possible $\by$ is bounded by the same argument by $|X|^{O(\log|X|)}$, since there are $O(\log |X|)$ points of $X$ in $\by$. 

Hence, the total size of $\cand$ is at most
$\exp\big( O(\log^2 |X| + z^4\eps^{-4} \log \eps^{-1} \log |X| )\big)$.

\paragraph*{Error analysis.}
We now show that for all solution $\calS$, every center can be approximated by a point of $\cand$. Let $S$ be some cluster of $\calS$, with center $s$. We show how to find $\tilde s \in \cand$ such that, for every $y \in X \cap S$ of type tiny or interesting, $|\cost(y, s) - \cost(y, \tilde s)| \leq 3\eps \left(\cost(y, s) + \cost(y, \greedy)\right)$.

For this, let $R_1, ..., R_{\log |X|}$ be the path in $\calR$ from the root to the leaf containing $s$, and $\{P^i_j\}$ be the paths given by \cref{lem:mf_sp_sep}.  For a point $p \in R_i, ~y \notin R_{i+1}$, we say that the path $P^i_j$ separates $p$ and $s$ if the path $p \leadsto s$ is fully contained in $R^i_j$ and intersect $P^i_j$.

For every region $R_i$ and path $P^i_j$, let $p^i_j \in R_i$ be the point separated from $s$ by the path $P^i_j$ with smallest $\cost(p^i_j, \greedy)$ value. Let $\by$ be the tuple $(p^1_1, p^1_2,..., p^2_1, p^2_2, ...)$, 
and $\tilde s$ be the point of $\cand$ that has the same rounded distance tuple to $\calL_\by$ than $s$. Let $\tilde \calS$ be the solution constructed from $\calS$ that way. We show now that $\tilde \calS$ has the required properties. As in \cref{lem:k2unionbound2} and \ref{lem:centroid-treewidth}, we first show that points close to $\calS$ are close to $\tilde \calS$, and the converse can be shown exactly the same way, by switching roles of $s$ and $\tilde s$.

For this, let $p \in X$ such that $\cost(p, \calS) \leq \left(\frac{10z}{\eps}\right)^z \cost(p, \greedy)$. We show that $\cost(p, \tilde \calS) \leq (1+\eps)\cost(p, \calS) + \eps \cost(p, \greedy)$.  Let $s$ be the closest center of $\calS$ to $p$.

Let $R_i$ be the smallest region containing the entire shortest-path between $p$ and $s$. If $R_i$ is a leaf, then $p \in \calL_\by$ and since $\dist(p, s) \leq \frac{4z}{\eps} \dist(p, \greedy)$,  the rounding of distances ensures that $\dist(s, \tilde s) \leq \frac{\epsilon}{z} \dist(p, \greedy)$ and so the cost satisfies $\cost(p, \tilde s) \leq (1+\eps)\cost(p, s) + \eps \cost(p, \greedy)$. Otherwise, there exists a path $P^i_j$ separating $p$ and $s$. Note that, by choice of $P^i_j$, $\dist(p, s) = \dist_{R^i_j}(p, s)$. As explained in the sketch of proof, we need to distinguish two cases.

\begin{itemize}
\item If $\dist_{R^i_j}(p, s) > \frac{8z^2}{\eps^2}\cdot \dist_{R^i_j}(p^i_j, s)$. Then we argue that $d(s, \tilde s)$ is negligible. By choice of $\tilde s$, $s$ and $\tilde s$ have the same rounded distance to $p^i_j$, i.e. $\dist_{R^i_j}(\tilde s, p^i_j) \leq \dist_{R^i_j}(s, p^i_j) + \frac{\eps}{z}\cdot \dist(p, \greedy)$ and so:
\begin{align*}
\dist(s, \tilde s) &\leq \dist_{R^i_j}(s, \tilde s) \leq 2 \dist_{R^i_j}(s, p^i_j) + \frac{\eps}{z}\cdot \dist(p, \greedy) \\
&\leq \frac{\eps^2}{4z^2} \dist(p,s) + \frac{\eps}{z}\cdot\dist(p, \greedy) \leq \frac{(1+\eps)\eps}{z} \cdot \dist(p, \greedy)
\end{align*}

Hence, using the modified triangle inequality as above, we have
:
\begin{align*}
\cost(p, \tilde s)  &\leq (1+\eps(1+\eps)) \cost(p, s) + (1+\nicefrac{z}{\eps(1+\eps)})^{z-1} \cost(s, \tilde s)\\
&\leq (1+\eps(1+\eps)) \cost(p, s) + (1+\eps)^2(\eps/z)\cost(p, \greedy)\\
&\leq (1+2\eps)\cost(p, s) + 2\eps\cost(p, \greedy).
\end{align*}


\item Otherwise, $\dist_{R^i_j}(p, s) \leq \frac{8z^2}{\eps^2}\cdot \dist_{R^i_j}(p^i_j, s)$ and we can make use of the landmarks. 
By definition of $j$, the path $y \leadsto s$ is entirely in $R^i_j$, and it crosses $P^i_j$ at some vertex $x$. 

First, it holds that $\dist_{R^i_j}(x, p^i_j) \leq \dist_{R^i_j}(x, s) + \dist_{R^i_j}(s, p^i_j) \leq \dist_{R^i_j}(p, s) + \dist_{R^i_j}(s, p^i_j) \leq (1+\frac{8z^2}{\eps^2})\dist_{R^i_j}(p^i_j, s) \leq \frac{9z^2}{\eps^2}\cdot \frac{10z}{\eps}\cdot \dist(p^i_j, \greedy)$, hence $x$ is in $P \cap B_{R^j_i}(p^i_j, \frac{90z^3}{\eps^3} \dist(p^i_j, \greedy))$. 
%\david{size of ball here}
By choice of landmarks, this implies that there is $l \in \calL_\by$, with $\dist(x, l) \leq \frac{\epsilon}{z} \dist(p^i_j, \greedy) \leq \eps \dist(p, \greedy)$. %\david{precision of the net here}
Furthermore, 
\begin{align*}
\dist_{R^i_j}(s, l) &\leq \dist_{R^i_j}(s, x) + \frac{\epsilon}{z} \cdot \dist(p^i_j, \greedy)  \leq \dist_{R^i_j}(p, s) + \frac{\epsilon}{z} \dist(p^i_j, \greedy) \\
&\leq \frac{8z^2}{\eps^2}\cdot \dist_{R^i_j}(p^i_j, s) + \frac{\eps}{z}\cdot\dist(p^i_j, \greedy)\\
&\leq (\frac{8z^2}{\eps^2} \cdot \frac{10z}{\eps} + \eps/z)\dist(p^i_j, \greedy).
\end{align*}
%$\dist_{R^i_j}(s, l) \leq \dist_{R^i_j}(y, s) + \eps\dist(p^i_j, \greedy) \leq \frac{8z^2}{\eps^2}\cdot \dist_{R^i_j}(p^i_j, s) + \eps\dist(p^i_j, \greedy) \leq (\frac{8z^2}{\eps^2} \cdot \frac{4z}{\eps} + \eps)\dist(p^i_j, \greedy)$.
Hence, $s$ is close enough to $l$ to ensure that $\tilde s$ has the same rounded distance to $l$ as $s$, and we get: 
\begin{align*}
\dist(p, \tilde s) & \leq \dist_{R^i_j}(p, l) + \dist_{R^i_j}(l, \tilde s) \\
&\leq \dist_{R^i_j}(p, l) + \dist_{R^i_j}(l, s) + \frac{\epsilon}{z}\cdot \dist(p, \greedy) \\
&\leq \dist_{R^i_j}(p, x) + \dist_{R^i_j}(x, s) + \frac{3\epsilon}{z}\cdot \dist(p, \greedy) \\
&= \dist_{R^i_j}(p, s) + \frac{3\epsilon}{z}\cdot\dist(p, \greedy)\\
&= \dist(p, s) + \frac{3\epsilon}{z}\cdot\dist(p, \greedy)
\end{align*}

We can therefore conclude : $\cost(p, \tilde \calS) \leq (1+3\eps)\cost(p, \calS) + 3\eps \cost(p, \greedy)$.
%\begin{align*}
%\left\vert\cost(p, \tilde s) - \cost(p, s)\right\vert &\leq 3\eps \cost(p, s) + (1+\nicefrac{z}{3\eps})^{z-1} (\frac{3\epsilon}{z})^z \cost(p, \greedy)\\
%&\leq  3\eps \cost(p, s)+ \eps \cost(p, \greedy).
%\end{align*}
\end{itemize}

Showing the converse, i.e., that for points $p \in X$ such that $\cost(p, \tilde \calS) \leq \left(\frac{10z}{\eps}\right)^z \cost(p, \greedy)$ it holds that$\cost(p, \calS) \leq (1+\eps)\cost(p, \tilde \calS) + \eps \cost(p, \greedy)$ is similar. As in \cref{lem:k2unionbound2}, this concludes the proof.

\end{proof}

